GraphIt: A High-Performance DSL for Graph Analytics

The performance bottlenecks of graph applications depend not only on the algorithm and the underlying hardware, but also on the size and structure of the input graph. Programmers must try different combinations of a large set of techniques to develop the best implementation for a specific algorithm and type of graph. Existing graph frameworks lack flexibility, supporting only a limited set of optimizations. This paper introduces GraphIt, a new DSL for graph computations that generates fast implementations for algorithms with different performance characteristics running on graphs with different sizes and structures. GraphIt separates what is computed (algorithm) from how it is computed (schedule). Programmers specify the algorithm using an algorithm language, and performance optimizations are specified using a scheduling language. The algorithm language simplifies expressing the algorithms. We formulate graph optimizations, including edge traversal direction, data layout, parallelization, cache, NUMA, and kernel fusion optimizations, as tradeoffs among locality, parallelism, and work-efficiency. The scheduling language enables programmers to easily search through this complicated tradeoff space by composing together optimizations. We also built an autotuner to automatically find high-performance schedules. The compiler uses a new scheduling representation, the graph iteration space, to model, compose, and ensure the validity of the large number of optimizations. GraphIt outperforms the next fastest of six state-of-the-art shared-memory frameworks (Ligra, Green-Marl, GraphMat, Galois, Gemini, and Grazelle) on 24 out of 32 experiments by up to 4.8$\times$, and is never more than 43% slower than the fastest framework on the other experiments. GraphIt also reduces the lines of code by up to an order of magnitude compared to the next fastest framework.

==> appendices.tex <==
\myparagraph{Fusing iterative graph kernels} Program
structure optimizations enable optimization across iterative graph kernels, such as
PageRank and Eigenvector Centrality as shown below.
\punt{(Listing~\ref{lst:kernel_fusion})}

\begin{lstlisting}[ label={lst:kernel_fusion}, language=graphit,escapechar=|]
...
func updateEdge(src : Vertex, dst : Vertex)
    NewRank[dst] += OldRank[src] / OutDegree[src];
end
func updateEdgeEigenVector(src : Vertex, dst : Vertex)
    NewEc[dst] += OldEc[src];
end
func main()
    #l1# for i in 1:10
        #s1# edges.apply(updateEdge);
        vertices.apply(updatePRVertex);
    end
    #l2# for i in 1:10
         #s1# edges.apply(updateEdgeEigenVector);
         vertices.apply(updateECVertex);
    end
end
schedule:
program->fuseFields({``OldRank'', ``OutDegree'', ``OldEc''})
->fuseForLoop(``l1'', ``l2'', ``l3'')
->fuseApplyFunctions(``l3:l1:s1'', ``l3:l2:s1'', ``fusedFunc'')
->configApplyParallelization(``l3:l1:s1'', ``vertex-parallel'')
->configApplyDirection(``l3:l1:s1'', ``DensePull'');
    
\end{lstlisting}


The goal is to fuse together the iterative kernels into a single
iterative kernel by fusing together the loops, functions, and 
vectors that are always accessed together (OldRank, OutDegree, and
OldEc) to significantly boost spatial locality.  
We use the command \fuseForLoop, which fuses
together two for-loops, identified by the labels \textbf{l1} and
\textbf{l2}, and replaces them with a new for-loop \textbf{l3}.  If
the index ranges of the original for-loops are not the same, two
additional for-loops, \textbf{l1\_prologue} and \textbf{l1\_epilogue},
will be generated to ensure the correctness of the program.  The fused
loop replace the original \textbf{l1} loop.  
The command \fuseApplyFunctions{} creates a
new edgeset \apply{} to replace the \textbf{l3:l1:s1} 
statement.  In Section~\ref{sec:eval}, we show that fusion of multiple
iterative kernels with similar access patterns can boost the
performance of the application by up to 60$\%$.


==> compiler_stash.tex <==
\punt{

across different source vertices (using a work-stealing runtime), 
but not across different edges within the same source vertex, as shown in the following snippet.
%% This is because there is enough parallelism at the outer for loop and parallelizing the inner loop would result in extra overhead.
%It leverages a work-stealing runtime to achieve good load balance.
\begin{lstlisting} [language = c++]
	parallel_for (NodeID src = 0; src < num_verts; src++) {
		for (NodeID dst : G.getOutNghs(src)){
			applyFunc(src,dst);} }
\end{lstlisting}

The edge-aware-vertex-parallel mode also parallelizes across different
source vertices. However, it partitions the vertex array based on the
number of edges. The partition of chunks can be done in a
divide-and-conquer mechanism. Below is pseudocode that illustrates the
new iteration space.

In the pull direction, vertex-parallel partitions the permuted graph
iteration space, exploiting parallelism across different destination
vertices as shown below.

\begin{lstlisting} [language = c++]
	parallel_for (NodeID dst = 0; dst < num_verts; dst++)
		for (NodeID src : G.getOutNghs(dst))
			applyFunc(src,dst); 
\end{lstlisting}
}


\punt{A key challenge is to automatically insert 
synchronizations for different combinations of direction and parallelization schemes. 
A \SparsePush \VertexParallel traversal needs different synchronizations than a \DensePull \VertexParallel traversal. }


\punt{

% \subsection {Schedule-Driven Optimization Pass Orchestration}
\subsection {Multiple Edge Traversal Optimizations Code Generation}
In order to support multiple edge traversals optimization, 
\graphit introduces a new schedule-driven optimization pass orchestration design that
allows users to add more optimization passes and dictate the order of
the added optimizations with the label-based scheduling language
described in Section~\ref{sec:schedule}. Users can perform fine-grained
loop fusion, loop splitting, and fusion of \apply{} functions on
loops and functions specified with statement labels and scheduling commands.

These optimizations are implemented as customized optimization passes
on the intermediate representation of the program. \graphit implements these
program structure transformation schedules by adding new optimization passes 
that transform the intermediate representation. 
To enable this flexibility in the optimization pass structure, \graphit compiler exposes a set of
restricted IR manipulation APIs and uses a dynamic mapping technique
between labels and IR nodes.  The restricted low-level APIs allow the
creation, removal, cloning, and fusion of certain types of IR nodes,
such as loops, \apply{} expressions, and functions.  The targets of these
low-level APIs are identified with labels.  The high-level scheduling
commands that split or fuse loops and functions are implemented with the low-level APIs.

}


\punt{

For example,  the schedule below
adds a new loop splitting optimization pass to the compiler by
invoking a function to transform the intermediate representation from
one loop (\textbf{l1}) to two separate loops (\textbf{l2} and \textbf{l3}).


\begin{lstlisting} [language=graphit, escapechar=|]
#l1# for i in 1:11
	#s1# edges.from(Frontier).apply(updateEdge);
end
schedule:
program
->splitForLoop("l1", "l2", "l3", 3, 7);
->configApplyDirection("l2:s1", "DensePull")
\end{lstlisting}
}

% \julian{the syntax of \splitForLoop is never defined}

\punt{
\begin{figure}[!h]
\includegraphics[width=0.7\columnwidth]{figures/schedule_driven_opt_orc}
\caption{Schedule-Driven Optimization Pass Orchestration}
\label{fig:schedule_driven}
\end{figure}
}


\punt{
In the example above, the apply operator lowering
pass would go into loop \textbf{l2} and computes the current scoped label
(\textbf{l2:s1}) for the \apply{} expression in the first split loop. The
compiler sees a match between current label and the label specified in
the second scheduling command, and proceeds to lower the \apply{}
expression with a \DensePull traversal configuration.

\julian{potentially remove the code example above}
\julian{defer stuff to the appendix.}
}

\punt {
%These scheduling commands are implemented as functions that take as input the  IR and modifies the IR directly.
The key challenge here is how to combine loop fusion and splitting with other optimizations. This requires maintaining the consistency of labels in the presence of fusion of loops. The original loop node is removed and a name node is created to replace the for loop node.  This would allow users to reference the newly created code using the old label.
}



\punt{





\subsection{Lowering Apply Modified Operators}
There are several components to generate code for the direction optimization, including inserting additional function declarations, adding modification tracking logic, generating the edge traversal code with filtering operators, and deduplication logic when adding vertices to the next frontier. 

% add some description on how this maps to graph iteration space here

First, the compiler changes the user-provided \apply function from returning nothing to returning a boolean value.  The compiler performs this if the field of the destination vertex, which is specified by the \textit{modified} keyword, is modified in the code. To do this transformation, we create a \textit{modified\_flag} for each assignment and reduction operator; this tag is initialized to false. When a field associated with the destination vertex is updated through an assignment or reduction operator, the \textit{modified\_flag} of the statement would be set to true. In the end, we insert a return statement that returns the \textit{modified\_flag} of the field specified by the user. 

In the following example, the \textit{apply\_f} function for connected components below initially returns no value. 

\begin{lstlisting}[language = graphit]
func apply_f (src:Vertex, dst:Vertex)
	component[dst] min= component[src];
end
\end{lstlisting}

Later, the program generates a \textit{component\_modified\_flag} to track the changes to the component field and returns the flag in the end, as shown in the following code. 

\begin{lstlisting} [language = c++]
bool apply_f(src:int, dst:int) {
	bool component_modified_flag = false;
	if (component[src] < component[dst]){
		component[dst] = component[src];
		component_modified_flag = true;}
	return component_modified_flag;}
\end{lstlisting}



Once the compiler has updated the user provided apply function with modification tracking logic, it needs to generate edge traversal code in the direction specified by the scheduling language. \graphit achieves this by generating different for loops traversing incoming edges and outgoing edges. 



\subsection{Runtime Libraries}

We built a runtime library for high performance data structures, including bitvector, vertexset, graph representation, and atomic synchronization primitives. The runtime code borrows heavily from libraries from both GAPBS~\cite{DBLP:journals/corr/BeamerAP15} and Ligra~\cite{shun13ppopp-ligra}. 
}

==> intro_stash.tex <==
% old text that was in intro
\punt{

Extracting information from
these graphs often involves running algorithms for identifying the
important vertices, finding connections among vertices, and detecting
communities of interest. Speeding up these applications can
enhance the efficiency of data analytics applications and improve
the quality of Web services. }

\punt{

 multiple
implementations of the same algorithm to identify the best combination
of optimizations for a specific algorithm and input data.

The optimized program often sacrifices clarity,
portability, and modularity for performance.

% leave this in the introduction
Because of this lack of performance flexibility, we found that none of the recent high-performance
graph frameworks can consistently perform within 6$\times$ of the fastest
framework for PageRank, Connected Components,
Breadth-First Search and Single Source Shortest Paths across
social networks, road networks and web graphs.

The algorithm is specified using high-level
 operators on vertex and edge sets.
}

\punt{
However, many performance-conscious
developers often still use hand optimized implementations or
new custom-built frameworks for their specific class of problem, instead of general purpose high-performance
graph systems~\cite{Sharma2016,Zhisong2017,Chantat2017}.
}
\punt {
	% For now, we don't show machine properties.
	machines with differing properties,
}

\punt{
Most of the existing graph frameworks focus on
developing new techniques that benefit a subset of applications and data sets,
instead of supporting efficient composition of existing optimizations as shown in Table~\ref{table:related-table}.
}

\punt{
While auto-tuning for the best combination of schedules is
a more attractive solution, our work is a first step toward this goal.
The separation of algorithm and schedule enables autotuners and autoschedulesr to be
built on top of the compiler; without this separation, and the guarantee that schedules do not affect correctness, it would be far more difficult to automatically choose a point in the optimization space for a specific algorithm.
Additionally, Halide~\cite{Ragan-Kelley:2013:HLC:2499370.2462176}, an image
processing DSL, has demonstrated that expert programmers prefer manual
control of performance optimizations over automatic optimizations when
obtaining the highest performance is a requirement.}

% Deprecated

\punt{
\item a schedule-driven optimization pass orchestration design that allows the schedule to add new optimization passes and specify their execution order (Section~\ref{sec:compiler}).
}

\punt{
The compiler achieves consistent high performance
by supporting efficient implementations of combinations of optimizations
proposed by different graph frameworks,
while exploring new combinations that have not been tried previously
\riyadh{no need to say the following "as shown in Table~\ref{table:related-table}"}.


Implementing an optimization
is done by specifying a few simple scheduling commands in
the code and does not change the algorithm



The \emph{scheduling
  language} allows users to easily
combine a space of execution order, data layout and program structure
optimizations that we identified from our experiences with hand optimizing graph applications and experimenting with different graph processing frameworks.
  Implementing an optimization is done by specifying a few
simple scheduling commands in the code without changing
the algorithm.  Trying different combinations of graph optimizations
can be done by simply changing the scheduling
commands.

In order to combine together and generate efficient and valid implementations of
the execution ordering optimizations,
we propose a formal model that we call the \emph{graph iteration space}.

We use this formal model to represent, combine
and reason about the validity of
optimizations.
It maps many graph optimizations to the classical concept of iteration space
developed for dense loops~\cite{wolf1991loop, padua1986advanced} and
leverages data dependence
analysis~\cite{maydan1991efficient,li1989data} to insert low-level
synchronization primitives for parallelization optimizations. The model
also enables new optimizations that fuse together multiple graph kernels.
We encode the model in the intermediate representations
in the compiler to generate the efficient implementations in the end.

}

\punt{
\riyadh{Replace "difficult to produce hundreds of combinations of operators and optimizations"
with "does not allow easy exploration of the large space of optimizations"}.
\riyadh{The previous argument is not strong against the use of libraries. The
reader might say: Ok if I have one application I can still spend lot of
resources on just optimizing that specific application. The usual and classical
arguments for DSLs are: they provide productivity, portability, better
performance through optimization, better performance through easy exploration
of the space of optimizations (which is the case of graphit).  Currently we
only use the last argument.}
}




\punt{
\item a compiler that can separate the algorithm from schedule and data layout descriptions and generate fast implementations by combining together these specifications.
\item a flexible scheduling language design that can map optimizations to elements in the program after program transformations.
\item a schedule-driven optimization pass orchestration design that allows the schedule to add new optimization passes and specify their execution order (Section~\ref{sec:compiler}).
\item a code generation framework that can compose together complex global program and data structure transformations used in graph optimizations (Section~\ref{sec:compiler}).
}

% Deprecated Texts


\punt{
% introducing the performance inconsistency
Graph frameworks are not widely adopted because they lack performance
generality: each framework works well on
 a subset of applications for specific types of input on specific machines, but can have suboptimal performance
 on applications with different characteristics, machines with differing properties, and graphs with different structures.
 Figure ~\ref{fig:intro_comparisons} shows that no single
 framework performs well across all applications on all types of input.
 \riyadh{Just remove the sentence in red, it is complicated to understand and looking at the graph make the preformance difference abvious.
     Can you make the caption of the graph clear so that anyone who looks at
	 the graph understands what are the numbers, the applications, ...}
 \yunming{In fact, no framework is
 consistently within 2x of the best performing frame work for all algorithms on all datasets.}
 Developers who \riyadh{"have performance critical applications" instead of
 "don't have a deep knowledge of the performance characteristics
 of the different frameworks"}, cannot afford to leave this much performance \riyadh{Remove "on the table"}
 for their latency sensitive applications.
 This \performanceInconsistency issue is not unique to a specific framework, as shown in previous studies~\cite{Satish14Sigmod} and in Section~\ref{sec:related}.
 }


\punt{


% The algorithm language
The algorithm language raises the level of abstraction to expose
opportunities for optimizations, while significantly simplifying the
expression of graph algorithms.  Vertex sets, edge
sets, and their associated data are expressed abstractly to enable
physical data layout optimizations. The high-level operators remove low-level
implementation details, separating edge filtering
logic from edge update logic to expose scheduling and data layout optimization opportunities.

% The scheduling language
The scheduling language and the compiler allow the programmer to
compose complex graph optimizations and generate efficient C++
implementations.  To achieve this goal, we first propose a new
scheduling representation that can allow the user to specify and
combine many execution order, data layout and program structure
optimizations easily.  The language can map optimizations to program
elements (loops, vertex and edge set operators, etc.), even after the
structure of the program changes drastically.  We also introduce a new
model, which we call \textit{graph iteration space}, to represent and compose
together various optimizations in the compiler.  The graph iteration space model
maps many graph optimizations to iteration space theory and practices
developed for dense loops~\cite{wolf1991loop, padua1986advanced}, and
leverages data dependence
analysis~\cite{maydan1991efficient,li1989data} to insert low-level
synchronization primitives for parallelization optimizations.
Finally, instead of using the traditional fixed compiler optimization
pass structure, \graphit presents a new design that allows users to
add customized optimization passes to support graph optimizations that
need fine-grained program transformations, such as
loop splitting and fusion.


}


\punt{
We argue that it is as important, if not more important, to come up with solutions that
 can support efficient composition of all the optimization techniques that
have shown to perform well in existing frameworks in a programmer-friendly package.
This would allow the users to explore a large space in the locality, parallelism and work tradeoff space.
}


\punt{
Graph applications are often memory
bound, doing very little computation per byte accessed. CPUs are
often stalled on high latency random DRAM accesses~\cite{Beamer15IISWC}.
Many techniques
have been proposed to improve the locality of the memory accesses~\cite{Kiriansky2016,Beamer2017,Satish14Sigmod}, to
take advantage of the multi-core architecture with parallelization,
and to reduce unnecessary work~\cite{Beamer-2012,shun13ppopp-ligra}.
However, these techniques can also
negatively impact the performance depending on the algorithm, the
hardware, and the data.
%% For example, using a bit-vector instead of a
%% boolean array to store binary information of vertices (e.g., whether a
%% vertex has been visited) can improve the spatial locality of memory accesses for
%% large graphs significantly.
%% However, the extra work to compress and
%% decompress the boolean array can outweigh the benefit on smaller
%% graphs.
Given this tradeoff space, programmers need to experiment with different
combinations of optimizations when they implement a new algorithm,
move to a new hardware platform, or handle data with a different
size and structure.
While the effects of graph optimization techniques have been known to expert programmers, one of the contributions of this paper is in framing the tradeoff space among locality, parallelism, and \work,
and describing how many graph optimizations fit into the space (Section~\ref{sec:tradeoff}).




% do we want to say  with limited performance tuning capabilities??
Various graph libraries
(e.g.,~\cite{shun13ppopp-ligra,zhang15ppopp-numa-polymer,sundaram15vldb-graphmat,nguyen13sosp-galois})
have been developed to reduce programming effort.
However, graph
libraries suffer from the inability to support and combine global program and data
structure transformations needed by many graph optimizations and
the lack of support for optimizations across multiple graph
kernels.
For example, data layout optimizations, which need to transform both
declarations and accesses points of vertex/edge data,
and
parallelization optimizations,
which need to add parallel constructs for loops or
tasks and insert synchronization instructions to the
appropriate read/write accesses, are both challenging for graph libraries to support.
Furthermore, graph applications often
involve multiple kernels that extract different properties of the graph,
such as different centrality measurements and the number of connected
components~\cite{leskovec2016snap}. Libraries have no support for
program structure transformations needed to optimize across multiple
kernels.


% I am not too sure what we want to write here.
Existing graph domain specific languages
(DSLs)~\cite{Hong12asplos,socialite13ICDE,Aberger2016} do not expose
comprehensive performance tuning capabilities to users and explore
limited set of points in the tradeoff space. These DSLs often cannot
take advantage of the expert programmers' knowledge needed for
selecting graph optimizations.  Previously,
Halide~\cite{Ragan-Kelley:2013:HLC:2499370.2462176}, an image
processing DSL, has demonstrated that expert programmers prefer manual
control of performance optimizations over automatic optimizations when
obtaining the highest performance is a requirement.  Compared to image
processing, graph applications require navigating a more complicated
performance tradeoff space and optimizing them requires implementing
more complex program and data transformations.


}


==> overview.tex <==
\section{\graphit Overview}
\label{sec:overview}

\punt{The optimized implementations get even more complicated with other applications that need additional optimizations and more operators, such as filtering on source or destination vertices (BFS) and tracking changes to vertex data (CC, SSSP).}

In Section~\ref{sec:tradeoff}, we show that it is very challenging to find the right combination of optimizations for graph algorithms. For PageRankDelta, you can easily come up with more than 30 optimized implementations (at least 5 directions, 3 parallelization strategies, vertex data layout optimization, cache optimization, and NUMA optimization). Different combinations require inserting different synchronization instructions and use different ways to create and reference the data structures. State-of-the-art libraries and DSLs have no way for the user to generate all these optimized implementations. Trying out these optimizations by hand becomes incredibly tedious for the developers and the final implementations are often hard to read and need to be discarded when moving to a new hardware platform or processing input with a different size and structure.

To tackle this challenge, we propose \graphit, a new graph DSL and compiler that leverages a high-level algorithm representation and a scheduling language to compose together graph optimizations, enabling comprehensive searches through a complicated tradeoff space between locality, parallelization and work efficiency. 
\graphit is built around the idea of decoupling what is computed (\textbf{algorithm}), from how it is computed (\textbf{schedule}), and how the data is stored (\textbf{physical data layout}).
The users describe the algorithm in the high level algorithm language and specify performance optimizations in the separate scheduling language. 
This separation of \emph{what} and \emph{how} simplifies the algorithm descriptions, enables users to easily experiment with a large combination of performance optimizations, leveraging their domain expertise to find the best schedule.



==> programming_asplos18.tex <==
\section{Language Design}
\label{sec:programming}

The \graphit DSL is built around the idea of decoupling
\emph{what} should be computed from \emph{how} to compute it. 
The users describe the algorithm in a high level language
(the \emph{algorithm language}) without providing
low level implementation details.
They specify performance optimizations in a separate language
which we call the \emph{scheduling language}. This separation of \emph{what} and \emph{how} simplifies the algorithm descriptions, enables users to easily experiment with a large combination of performance optimizations using the scheduling language, and leverages their domain expertise to find the best schedule. 




\punt{Sections~\ref{sec:algo_lang} and~\ref{sec:schedule_lang} describe the algorithm and scheduling languages in more detail. Section~\ref{sec:lang_example} shows a few applications written in \graphit.}


\punt{
The \emph{what} is the pure algorithm that should be computed
(without any optimization) while the \emph{how} is the set of
code and data layout transformations that should be applied
on the algorithm in order to get the best performance.
}

\punt{
% I am not sure where to put it 
Current compilers for general-purpose languages have a limited
ability to optimize graph applications, mainly because these
applications are expressed in languages such as C/C++ using
pointers.
An effective optimization requires an accurate dependence
analysis, which in turn requires an accurate alias analysis.
But in languages that permit recursive data structures
(multilevel pointer indirection), alias analysis is
undecidable~\cite{Landi:1992:USA:161494.161501,Ramalingam:1994:UA:186025.186041,pencil},
precluding success.
The \graphit compiler avoids this problem thanks to two design
choices: first, the \graphit DSL does not have pointers; this
eliminates all the aliasing problems that general purpose
compilers have; and second, the \graphit compiler does not
rely heavily on dependence analysis to decide whether different
apply functions can be run in parallel; such an information
is provided by the user (yet the compiler still needs to
analyse the code to find out the shared variables and
transform them into atomic instructions, but this is
easier in a pointer-free language).
}

\subsection{Algorithm language}
\label{sec:algo_lang}

The \graphit algorithm language is designed to be expressive enough to specify a variety of algorithms, while exposing opportunities for performance optimizations. To do this, it is designed to be
\begin{denseitemize}
\item Highly Expressive : \graphit provides a small set of operators that can be composed to express a large class of graph applications. It can also handle applications involving multiple graphs with different type of vertices and edges.
\item Easy to Use: The user does not need to specify low level details such as atomic synchronizations, deduplication, and other performance optimization strategies, since \graphit has a separate scheduling language. \graphit also leverages compiler analysis and code generation to support language functionalities, such as tracking of updated vertices.  
\item Physical Data Independence: Vertex data and graphs are all stored in abstract vectors and sets with no implications on the underlying storage format. 
\item Parallelization Friendly: Set operations, such as \apply, expose data parallelism within the algorithm.  
\item Direction Optimization Ready: \graphit proposes new \from, \too, and \apply set operators that the compiler can use to automatically generate parallel direction optimized implementations.
\end{denseitemize}

The language is an imperative language centered on sets (vertexsets and edgesets) and operations on the sets. The user first defines element types and vectors associated with the element types. Then vertexsets and edgesets of elements are constructed and applications are mostly written using operators on vertexsets and edgesets. 


\subsubsection{Data Types} ~\\
In \graphit, the user defines vertex and edge element types at the beginning (Vertex and Edge in Figure~\ref{fig:code:bellmanford} line 1-2). Once the elements are defined, the user can add fields to the elements using vectors (SP in Figure~\ref{fig:code:bellmanford} line 5). Sets of vertices and edges are organized into built-in vertexset and edgeset types.

\begin{table}[t]
\footnotesize
 \begin{tabular}{p{2cm}p{4cm}}
\textbf{Data Type}  & \textbf{Example} \\
 \texttt{element} & \lstinline|element Vertex end;|\\ 
 \texttt{vector} & \lstinline|rank : vector (Vertex)[float] = 0;|\\ 
 \texttt{vertexset} & \lstinline|var vertices : vertexset {Vertex}; | \\ 
\texttt{edgeset} & \lstinline|var edges : edgeset {Edge}(Vertex, Vertex); |\\
\noalign{\smallskip}
  \end{tabular}
  \caption{\graphit Data Types}
  \label{table:data_types}
\end{table}

\punt{
\julian{What are the ``Vertex'' and ``Edge'' types? Should we say ``(e.g. integers, strings, etc.)''?}}

Table~\ref{table:data_types} shows examples of the \graphit data types. The user can define customized element types for different types of vertices and edges. A graph application can have multiple types of vertices and edges. The element is similar to a struct type in C or C++, without any field declaration. The \textbf{vector} type is used as a field of an element, similar to the field of a struct in C or C++. At the same time, it can also be processed as a separate vector.  The declaration \lstinline{rank : vector (Vertex)[float] = 0} indicates that rank is a field associated with the element type Vertex, and each element of the vector is of type float. Vector definitions abide by the physical data independence property. The underlying implementation can be a single array, a dictionary, or even a field of a struct in an array of structs.


A \textbf{vertexset} is a set of vertices, where each vertex can be used to index into a vector associated with the element type. \lstinline|var vertices : vertexset {Vertex}; | declares a new vertexset that consists of Vertex elements. The vertexset can be implemented as an array containing the vertices, or a number of vertices size boolean array or bitvector, where vertices in the set is marked as 1. Vertexsets can be created dynamically or extracted from an edgeset. 


An \textbf{edgeset} is a set of edges, where each edge has a source and a destination. An undirected graph would be represented by duplicating the directed edges.  The types of the source and destination vertices is indicated between parentheses (Vertex in the example). The source and destination vertices do not have to be of the same type. \lstinline|var edges : edgeset {Edge}(Vertex, Vertex); | declares a new edgeset with both end points of type Vertex. The edgeset can be implemented as Compressed Sparse Row (CSR) or Compressed Sparse Column (CSC) format. 

\punt{ \julian{do you mean Compressed Sparse Column Format? What about edge list format?} Currently edge list is not supproted}

\subsubsection{Language Constructs and Operators} ~\\
\graphit focuses on set operations, but also supports traditional language constructs such as \textit{for}, \textit{while}, and \textit{if} with some restrictions. 

\graphit provides various operators on the vertexsets and edgesets, as listed in Table~\ref{table:set_api}. The \from and \too operators are evaluated lazily when combined with an \apply operator. \textit{for} and \textit{while} loop can only be used in iterative applications. They cannot be used to traverse vertexsets or edgesets. This is enforced by making sure that graph traversal can be done only through the \apply operator. \textit{if} statements are used to express \emph{control flow} in the iterative graph applications. They cannot be used inside \apply functions as this would prevent the compiler from performing many performance optimizations. Instead, filtering can be expressed through a combination of \from, \too, and \textit{filter} operators. 

\begin{table*}[t]
\footnotesize
 \begin{tabular}{p{4.5cm}p{1.5cm}p{10.5cm}}
\textbf{Set Operation}  & \textbf{Return Type} & \textbf{Description} \\
 \texttt{vertices.filter(func)} & vertexset & filters out vertices where func(vertex) returns true\\ 
 \texttt{vertices.apply(func)} & vertexset & applies func(vertex) to every vertex and returns the entire vertexset \\ 
 \texttt{edges.filter(func)} & edgeset & filters out edges where func(edge) returns true\\ 
 \texttt{edges.from(vertexset)} & edgeset & filters out edges whose source vertex is in the vertexset\\ 
 \texttt{edges.to(vertexset)} & edgeset & filters out edges whose destination vertex is in the vertexset\\ 
 \texttt{edges.from(func)} & edgeset & filters out edges where func(source) returns true\\ 
 \texttt{edges.to(func)} & edgeset & filters out edges where func(destination) returns true\\ 
 \texttt{edges.apply(func)} & vertexset & applies func(source, destination) to every edge and returns the entire vertexset \\ 
 \texttt{edges.apply(func).modified(vect)} & vertexset & applies func(source, destination) to every edge. It returns a vertexset that contains destination vertices whose field vector has been modified in the edge apply operation \\ 
 \texttt{edges.getVertices()} & vertexset & returns a vertexset that contains the union of source and destination vertices \\
\noalign{\smallskip}
  \end{tabular}
  \caption{Vetexset and Edgeset API}
  \label{table:set_api}
\end{table*}




\subsection{Scheduling language}
\label{sec:schedule_lang}


\begin{table*}[t]
\footnotesize
 \begin{tabular}{p{8.0cm}p{12.5cm}}
\textbf{Schedules}  & \textbf{Optimization} \\
 \texttt{program->configApply(label, config)} & direction optimization\\ 
 \texttt{program->fuseFields(\{vect1,vect2,..\})} & physical data layout optimization\\ 
 \texttt{program->fuseForLoop(label1,label2,fused\_label)} & loop fusion (used in multi-kernel optimization)\\ 
 \texttt{program->splitForLoop(label, label1,label2,range)} & enables applying different optimizations for different iterations of the application \\ 
 \texttt{program->fuseApplyFunctions(label1,label2,fused\_func)} & fuse together two edgeset apply operators (used in multi-kernel optimization)\\ 
\noalign{\smallskip}
  \end{tabular}
  \caption{Scheduling Language API}
  \label{table:schedule_api}
\end{table*}


%Talk about the naming scope for label nodes, how to uniquely identify a statement 

The scheduling language provides users with the ability to explore a wide range of optimizations and an easy way to compose those optimizations for better performance. Supported optimizations include parallelism, physical data layout transformations, fusion of loops, and edgeset operations.  Table~\ref{table:schedule_api} summarizes the different scheduling commands. 

%const old_rank : vector{Vertex}(float) = 1.0/vertices.size();
%const new_rank : vector{Vertex}(float) = 0.0;
%const old_ec : vector{Vertex}(float) = 1.0/vertices.size();
%const new_ec : vector{Vertex}(float) = 0.0;
%const out_degree : vector {Vertex}(int) = edges.getOutDegrees();
%const error : vector{Vertex}(float) = 0.0;
%const damp : float = 0.85;
%const beta_score : float = (1.0 - damp) / vertices.size();

\begin{figure}[h!t]
\begin{lstlisting} [language=graphit]
...
func updateEdge(src : Vertex, dst : Vertex)
    new_rank[dst] += old_rank[src] / out_degree[src];
end
func updateEdgeEigenVector(src : Vertex, dst : Vertex)
    new_ec[dst] += old_ec[src];
end
func updatePRVertex(v : Vertex)
    new_rank[v] = beta_score + damp*(new_rank[v]);
    error[v] = fabs(new_rank[v] - old_rank[v]);
    old_rank[v] = new_rank[v];
    new_rank[v] = 0.0;
end
func updateECVertex(v : Vertex)
    old_ec[v] = new_ec[v];
    new_ec[v] = 0.0;
end
func main()
    #l1# for i in 1:10
        #s1# edges.apply(updateEdge);
        vertices.apply(updatePRVertex);
    end
    #l2# for i in 1:10
         #s1# edges.apply(updateEdgeEigenVector);
         vertices.apply(updateECVertex);
    end
end
schedule:
program->fuseFields({"old_rank", "out_degree", "old_ec"})
->fuseForLoop("l1", "l2", "l3")
->fuseApplyFunctions("l3:l1:s1", "l3:l2:s1", "fused_kernel")
->configApply("l3:l1:s1", "parallel")
->configApply("l3:l1:s1", "pull");
    
\end{lstlisting}
\caption{\graphit code fragment (before fusion)}
\label{fig:code:before_fusion}

\punt{

func updatePRVertex(v : Vertex)
    vector_struct[v].new_rank = 
    	beta_score + damp*(vector_struct[v].new_rank);
    vector_struct[v].error = 
    	fabs(vector_struct[v].new_rank - vector_struct[v].old_rank);
    vector_struct[v].old_rank = vector_struct[v].new_rank;
    vector_struct[v].new_rank = 0.0;
end

func updateECVertex(v : Vertex)
    vector_struct[v].old_ec = vector_struct[v].new_ec;
    vector_struct[v].new_ec = 0.0;
end
}
\begin{lstlisting} [language=graphit]
...
func fused_kernel(src : Vertex, dst : Vertex)
    vector_struct[dst].new_rank += 
    	vector_struct[src].old_rank / vector_struct[src].out_degree;
    vector_struct[dst].new_ec += vector_struct[src].old_ec;
end
... updatePRVertex and updateECVertex  ... 
func main()
    #l3# for i in 1:10
    	#l1# namenode
            #s1# edges.apply(fused_kernel);
            vertices.apply(updatePRVertex);
        end
        #l2# namenode
            #l1 vertices.apply(updateECVertex);
        end
    end
end 
\end{lstlisting}
\caption{\graphit code fragment (after fusion)}
\label{fig:code:fusion}
\end{figure}


Labels (\textbf{\texttt{\#label\#}} ) are used to identify targets of optimizations (i.e., the statements on which optimizations apply). Users can assign a label on the left side of a statement, and later reference it in the scheduling language.  The use of labels in this way is challenging because after the application of a scheduling command, new statements would be created or removed (meaning that new labels would also be created or removed).  For example, loop fusion would create a new loop, while destroying two old loops, as shown in Figure~\ref{fig:code:fusion}. To address these issues, we propose a scoped label scheme, i.e., labels have a scope and this original scope remains with the label even after the application of a sequence of scheduling commands.  In Figure~\ref{fig:code:before_fusion}, the first \apply operator (line 20) would be referenced as \textbf{l1:s1} instead of just \textbf{s1}. This is because \textbf{s1} falls under the naming scope of \textbf{l1}. If \textbf{l1} is not defined, then \textbf{s1} does not need a name scope. In the fusion example, the loop would be replaced as a name node with \textbf{l1} label. This enables the user to reference the first edgeset apply as \textbf{l3:l1:s1} and apply other optimizations on the target.

The built-in command \textit{ConfigApply} enforces a series of configurations to an \apply operation. The configurations fall into three different categories: edge traversal direction, deduplication, and parallelization configurations. The user can pick one configuration from each category and combine them to form the final apply operator configuration. 

The edge traversal configuration can be one of the following: \texttt{push}, \texttt{pull}, \texttt{hybrid\_dense\_forward}, or \texttt{hybrid\_dense}. Push performs a filtering on the source vertex (if the \from operator is used), and then goes through each outgoing edge, processing an edge with the apply function if the destination vertex fits the filtering criteria (if the \too operator is used). Pull performs a filtering on the destination vertex (if the \too operator is used), and then go through each incoming edge, process an edge with the apply function if the source vertex fits the filtering criteria (if the \from operator is used). \texttt{Hybrid\_dense\_forward} performs a check on the sum of outdegree of the current frontier. If the outdegree sum is greater than a threshold, then a dense forward version is used, where the direction is push, but the frontier is implemented as a boolean array. If the outdegree sum is less than the threshold, then the regular push is used. \texttt{Hybrid\_dense} performs a check on the sum of outdegree of the current frontier. If the outdegree sum is greater than a threshold, then the pull edge traversal with a pull apply function are used. Otherwise, the push edge traversal with a push apply function are used.

Deduplication can be configured with \texttt{enable\_deduplication} or \texttt{disable\_deduplication}. Enabling deduplication makes sure that no destination vertex would be added to the frontier twice. Disabling deduplication can save some runtime overhead when the user knows the application would not add the same destination vertex to the next frontier multiple times (e.g., in BFS). 

Finally, parallelization can be specified using the \texttt{serial} or \texttt{parallel} configurations. Synchronization primitives are automatically added to the programs. 


The built-in command \textit{FuseFields} fuses together multiple field vectors using an array of struct. This is critical for applications that access multiple fields of the same vertex via random access. For example, in the pull version of PageRank, the field vectors \texttt{old\_rank} and \texttt{out\_degree} are read from the source vertex via random access. By using an array of struct, the program can reduce random access by 2$\times$.

The command \textit{FuseForLoop} fuses together two for loops, identified by label1, label2, and replaces them with a new loop identified by \texttt{fused\_label}. If the index ranges of the original for loops are not the same, two additional for loops, \texttt{fused\_label\_prologue} and \texttt{fused\_label\_epilogue}, would be generated to ensure the correctness of the program. The fused loops would be inserted before the position of the original label1 loop. 

\punt{

, \texttt{fused\_label\_prologue}, \texttt{fused\_label\_epilogue}
}

\punt{ \julian{what are the prologue and epilogue loops?} }

The command \textit{SplitForLoop} splits the original for loop, identified by label, into two separate for loops, \texttt{split\_label1} and \texttt{split\_label2}. The first split loop's range goes from the lower of the original range to lower + split\_range, and the second goes from lower + split\_range to upper of the original range. This is useful for applications where the computation characteristics change as the computation progresses. The user can split up the graph kernel into two separate kernels, and provide different scheduling commands for both.

The command \textit{FuseApplyFunctions} fuses the apply function of two edgeset apply operations identified by label1 and label2. The new apply function would be named fused\_func. The new edgeset apply operation would replace the label1 statement. 



\subsection{Examples}
\label{sec:lang_example}

We demonstrate the ease of use of the algorithm language by comparing the \graphit and Ligra implementations of Bellman-Ford for single-source shortest paths. We also show and the flexibility of the scheduling language using an example of fusing together PageRank and Eigenvector Centrality. 

\textbf{BellmanFord} computes the shortest distance from source vertex (vertex 0) to all other vertices. At every iteration of the while loop, the distance to the current node is updated if the distance to the neighbor node plus the weight of the edge is smaller, as shown in Figure~\ref{fig:code:bellmanford}, line 7 for \graphit. 

	In the Ligra implementation (Figure~\ref{fig:code:ligra_bellmanford}), the user has to specify both a push and pull functions (lines 6 and 12), provide atomic synchronization primitives (lines 14--15) and make sure that the same destination node is not added to the frontier twice (lines 10, 15, 17--22). \graphit implementation (Figure~\ref{fig:code:bellmanford}) only needs to use the \textit{min=} reduction operator in line 7 to update \textit{SP[dst]}, a modified keyword to track changes to the \textit{SP} field vector, and a scheduling command to enable deduplication. 

\textbf{PageRank and EigenVector Centrality Fusion} PageRank and EigenVector Centrality aggregates neighbors' contribution (\textit{old\_rank/out\_degree}) and eigenvector centrality (\textit{old\_ec}) to update its own rank and eigenvector centrality. Both algorithms iteratively apply the aggregation for a fixed number of iterations. Part of the code is shown in Figure~\ref{fig:code:before_fusion}.

These two iterative kernels can be fused together in \graphit to reduce the total number of random reads on the neighbor's values (Figure~\ref{fig:code:fusion}). \graphit first fuses together the fields \textit{old\_rank}, \textit{out\_degree}, and \textit{old\_ec} using the \textit{fuseFields} command, ensuring that the physical layout will be an array of struct. Then it fuses the two outer for loops, \textbf{l1} and \textbf{l2} into a new for loop \textbf{l3}. The original for loops get replaced into two name nodes that are used to keep the label scope consistent. The first and second edgeset apply operator can be referenced using \textbf{l3:l1:s1} and \textbf{l3:l2:s1}. FuseApply fuses together the two edgeset apply operations within the newly formed \textbf{l3} loop and creates a new edgeset apply operator that replaces \textbf{l3:l1:s1}. The last two commands configures the fused edgeset apply operation to be parallel and works in the pull direction. 

\begin{figure}[t]
\begin{lstlisting} [language=graphit]
element Vertex end
element Edge end
const edges : edgeset{Edge}(Vertex,Vertex, int) = load (argv[1]);
const vertices : vertexset{Vertex} = edges.getVertices();
SP : vector{Vertex}(int) = 2147483647;
func updateEdge(src : Vertex, dst : Vertex, weight : int)
     SP[dst] min= (SP[src] + weight);
end
func main()
    var n : int = edges.getVertices();
    var frontier : vertexset{Vertex} = new vertexset{Vertex}(0);
    frontier.addVertex(0); %add source vertex
    SP[0] = 0;
    var rounds : int = 0;
    while (frontier.getVertexSetSize() != 0)
        #s1# frontier = edges.from(frontier)
        .apply(updateEdge).modified(SP);
	    rounds = rounds + 1;
    	if rounds == n
	        break;
	    end
    end
end
schedule:
program->configApply("s1","hybrid_dense_forward")
	->configApply("s1","parallel")
	->configApply("s1","enable_deduplication";
\end{lstlisting}
\caption{\graphit code fragment for Bellman-Ford}
\label{fig:code:bellmanford}
\end{figure}


%  long start = P.getOptionLongValue("-r",0);
%  long n = GA.n;
%  intE* ShortestPathLen = newA(intE,n);
%  {parallel_for(long i=0;i<n;i++) ShortestPathLen[i] = INT_MAX/2;}
%  ShortestPathLen[start] = 0;
%  int* Visited = newA(int,n);
%  {parallel_for(long i=0;i<n;i++) Visited[i] = 0;}
%  vertexSubset Frontier(n,start); //initial frontier
%  long round = 0;

%  Frontier.del(); free(Visited);
%  free(ShortestPathLen);
\begin{figure}[t]
\begin{lstlisting}[language=c++]
struct BF_F {
  intE* ShortestPathLen;
  int* Visited;
  BF_F(intE* _ShortestPathLen, int* _Visited) : 
    ShortestPathLen(_ShortestPathLen), Visited(_Visited) {}
  inline bool update (uintE s, uintE d, intE edgeLen) { 
    intE newDist = ShortestPathLen[s] + edgeLen;
    if(ShortestPathLen[d] > newDist) {
      ShortestPathLen[d] = newDist;
      if(Visited[d] == 0) { Visited[d] = 1 ; return 1;}}
    return 0;}
  inline bool updateAtomic (uintE s, uintE d, intE edgeLen){
    intE newDist = ShortestPathLen[s] + edgeLen;
    return (writeMin(&ShortestPathLen[d],newDist) &&
	    CAS(&Visited[d],0,1));}
  inline bool cond (uintE d) { return cond_true(d); }};
struct BF_Vertex_F {
  int* Visited;
  BF_Vertex_F(int* _Visited) : Visited(_Visited) {}
  inline bool operator() (uintE i){
    Visited[i] = 0;
    return 1;  }};
template <class vertex>
void Compute(graph<vertex>& GA, commandLine P) {
 ... set up data structures ... 
  while(!Frontier.isEmpty()){
    if(round == n)
      break;
    vertexSubset output = edgeMap(GA, Frontier, 
    	BF_F(ShortestPathLen,Visited), GA.m/20, DENSE_FORWARD);
    vertexMap(output,BF_Vertex_F(Visited));
    Frontier.del();
    Frontier = output;
    round++;  }
...}
\end{lstlisting}
\caption{Ligra code fragment for Bellman-Ford}
\label{fig:code:ligra_bellmanford}
\end{figure}

%\subsection{Correctness}
%\label{sec:lang_correctness}

%\graphit does not check whether the application of a specific scheduling
%command is correct.  Making sure that scheduling commands are applied correctly
%is the responsability of the user.
%This is similar to OpenMP for example where parallelizing a loop that
%should not be parallelized does not raise any compilation error.

% we provide the user with a set of scheduling commands that can
% transform the code in multiple ways.  When a user applies a scheduling command,

%For example, if a user fuses two loops and fusion in that context is not legal,
%i.e., it is incorrect to fuse them because of backward dependence between the
%two loops (the second loop reads a value produced by the last iteration of
%the previous loop), in this case the use of the fusion scheduling command
%yields the generation of an incorrect code.
%Currently, we do not provide any warning or error message in this case.

\punt{
\begin{figure}[h!t]
\begin{lstlisting} [language=graphit]
element Vertex end
element Edge end
const edges : edgeset{Edge}(Vertex,Vertex) = load (argv[1]);
const vertices : vertexset{Vertex} = edges.getVertices();
const IDs : vector{Vertex}(int) = 1;
func updateEdge(src : Vertex, dst : Vertex)
    IDs[dst] min= IDs[src];
end

func init(v : Vertex)
     IDs[v] = v;
end

func main()
    var n : int = edges.getVertices();
    var frontier : vertexset{Vertex} = new vertexset{Vertex}(n);
    vertices.apply(init);
    while (frontier.getVertexSetSize() != 0)
        #s1# frontier = edges.from(frontier)
        .apply(updateEdge).modified(IDs);
    end
end

schedule:
program->setApply("s1", "hybrid_dense")->setApply("s1", "parallel");
\end{lstlisting}
\caption{\graphit code fragment for connected components}
\label{fig:code:cc}
\end{figure}
}








==> schedule_lang_stash.tex <==
\punt{
\graphit's algorithm language imposes no constraints on the order of
traversing the edges and the physical layout of data structures.  
}


\punt{
As we saw in
Section~\ref{sec:tradeoff}, decisions such as the edgeset traversal direction,
parallelization strategy, cache and NUMA based graph partitioning,
 and vertex data layout can drastically affect performance.
%% These choices are critical to achieving good performance and should not affect the correctness of the algorithms. 
%% This set of choices determines how the values are computed (\textbf{schedule}) and how data are stored (\textbf{data layout}) for a graph algorithm.
These choices are bound by a fundamental tension among locality, \work, and
parallelism.  \graphit's scheduling language provides users
with the ability to explore a wide range of optimizations and an easy
way to compose optimizations for better performance.
}

% try not to change this paragraph, it was tricky to make sure no 
% scheduling commands overextend

\punt {
\graphit's scheduling language API (shown in Table~\ref{table:schedule_api})
allows the users to try out combinations of Single Edge Traversal, 
Vertex Data Layout, and Multiple Edge Traversal Optimizations. 
For Single Edge Traversal Optimizations, 
the compiler uses the high-level scheduling APIs to configure the graph iteration 
space vectors and tags. 
\configApplyDirection{} allows the user to configure 
the \outerIter, \innerIter 
(push would be src,dst and pul would be dst, src), 
along with the filtering on the \outerIter (\SparsePush uses Sparse Array filtering  
and \DensePush is Dense Bool Array filtering on the \outerIter).
Hybrid directions, such as \SparsePush-\DensePull, would create two set graph iteration 
space vectors and tags. Each graph iteration space vector and its tags can be configured separately 
with an optional direction argument. 
If no direction is specified, the command would configure both 
directions for hybrid directions. 
\configApplyDataStructure{} configures the Filtering Tag of the \innerIter.
\configApplyParallelization{} sets the Parallelization and Partition Tags for \BSG. 
\configApplyNumSSG{} creates the \SSG dimension and sets the Partition Tag. 
\configApplyNuma{} sets the Parallelization Tag for the \SSG dimension. 
Data layout optimizations change the layout of
vectors, which are vertex data(\fuseFields). 
Multiple edge traversal optimizations change
the structure of the original \graphit program (splitForLoop,
\fuseForLoop, and \fuseApplyFunctions). 
}


 \punt{
  and multiple edgeset traversals optimizations
 
 }

\punt{
The user picks the traversal method that generates the
smallest number of random memory accesses
(\configApplyDirection) and select the parallelization scheme
that achieves the most scalable performance
(\configApplyParallelization) depending on the traversal mode and
characteristics of the application. The user can also configure the
data layout of the vertexset used as an argument to \from{} and \too{}
operators, which we call the active set, with
configApplyDataStructure.  
For applications such as breadth-first search, the
\applyModified{} operator will not add duplicated nodes to the output
vertexset. As a result, the user can choose to disable deduplication
(\configApplyDeduplication).  The 
traversal and parallelization configurations are listed in
Table~\ref{table:schedule_api}, and described in
Section~\ref{sec:tradeoff}.  The default configuration for each category in Table~\ref{table:schedule_api} is shown in bold.
}


\punt{
% describe the challenges of the scheduling language 
\subsection{Scheduling Multiple Edge Traversal Optimizations}
\label{subsec:structural}



\myparagraph{Scoped Labels and Name Nodes} To compose multiple edge traversal
optimizations with single edge traversal and vertex data layout optimizations, we
designed the labels to be scoped and introduce a special name node to
allow the labels to function even after complex program
transformations. 

For example, in Listing~\ref{lst:loop_fusion}, in order to fuse together the 
two edge traversals, we first need to fuse together the two for loops. 
Loop fusion would create a new loop (\textbf{l3}), while destroying the two
old loops (\textbf{l1} and \textbf{l2}). Now, it would be difficult if
we want to schedule the first edgeset \apply{} operator in the
\textbf{l3} loop as the original loops \textbf{l1} and \textbf{l2} have
been removed from the program and both edgeset \apply{} operators have
\textbf{s1} as their label.  To address this, we first propose
a scoped label scheme, i.e., labels have a scope. The first \apply{}
operator (Line~\ref{line:fusion_first_apply} of
Listing~\ref{lst:loop_fusion}) has label \textbf{l1:s1}.  
This is because \textbf{s1} falls under
the naming scope of \textbf{l1}. If \textbf{l1} is not defined, then
\textbf{s1} does not need a name scope.  We also need a
name node, which only enforces a name scope for the label. 
Loop \textbf{l1} would be replaced with a name
node with the label \textbf{l1} (Line~\ref{line:name_node} of
Listing~\ref{lst:after_fusion}).  This enables the user to reference
the first edgeset \apply{} as \textbf{l3:l1:s1} and apply other
optimizations on the target as shown in
Line~\ref{line:schedule_fusion} of Listing~\ref{lst:loop_fusion}. We show an 
example fusing together Eigenvector Centrality and PageRank in the appendix. 
%% Next we show 
%% how this scoped label design can be used in kernel fusion and split optimizations.


\begin{lstlisting} [caption={GraphIt loop fusion}, label={lst:loop_fusion}, language=graphit, escapechar=|]
#l1# for i in 1:10 
     #s1# edges.apply(func1); |\label{line:fusion_first_apply}|
end
#l2# for i in 1:10
     #s1# edges.apply(func2);
end
schedule:
program->fuseForLoop("l1", "l2", "l3")
->configApplyDirection("l3:l1:s1", "SparsePush"); |\label{line:schedule_fusion}|
\end{lstlisting}
%\caption{\graphit code for fusion}
%\label{fig:code:before_fusion}

\begin{lstlisting} [caption={Pseudocode after fusion}, label={lst:after_fusion}, language=graphit,escapechar=|]
#l3# for i in 1:10
    #l1# namenode |\label{line:name_node}|
         #s1# edges.apply(func1); 
    end
    #l2# namenode
         #s1# edges.apply(func2);
    end
end
\end{lstlisting}
% \caption{pseudo code after fusion}
% \label{fig:code:after_fusion}
% \end{figure}

% moved to appendix 
\myparagraph{Fusing iterative graph kernels} Program
structure optimizations enable optimization across iterative graph kernels, such as
PageRank and Eigenvector Centrality as shown below.
\punt{(Listing~\ref{lst:kernel_fusion})}

\begin{lstlisting}[ label={lst:kernel_fusion}, language=graphit,escapechar=|]
...
func updateEdge(src : Vertex, dst : Vertex)
    NewRank[dst] += OldRank[src] / OutDegree[src];
end
func updateEdgeEigenVector(src : Vertex, dst : Vertex)
    NewEc[dst] += OldEc[src];
end
func main()
    #l1# for i in 1:10
        #s1# edges.apply(updateEdge);
        vertices.apply(updatePRVertex);
    end
    #l2# for i in 1:10
         #s1# edges.apply(updateEdgeEigenVector);
         vertices.apply(updateECVertex);
    end
end
schedule:
program->fuseFields({"OldRank", "OutDegree", "OldEc"})
->fuseForLoop("l1", "l2", "l3")
->fuseApplyFunctions("l3:l1:s1", "l3:l2:s1", "fusedFunc")
->configApplyParallelization("l3:l1:s1", "vertex-parallel")
->configApplyDirection("l3:l1:s1", "DensePull");
    
\end{lstlisting}


The goal is to fuse together the iterative kernels into a single
iterative kernel by fusing together the loops, functions, and 
vectors that are always accessed together (OldRank, OutDegree, and
OldEc) to significantly boost spatial locality.  
We use the command \fuseForLoop, which fuses
together two for-loops, identified by the labels \textbf{l1} and
\textbf{l2}, and replaces them with a new for-loop \textbf{l3}.  If
the index ranges of the original for-loops are not the same, two
additional for-loops, \textbf{l1\_prologue} and \textbf{l1\_epilogue},
will be generated to ensure the correctness of the program.  The fused
loop replace the original \textbf{l1} loop.  
The command \fuseApplyFunctions{} creates a
new edgeset \apply{} to replace the \textbf{l3:l1:s1} 
statement.  In Section~\ref{sec:eval}, we show that fusion of multiple
iterative kernels with similar access patterns can boost the
performance of the application by up to 60$\%$.
}

\punt{

  To do this, \graphit provides the 
command \splitForLoop, which splits the original for-loop, identified
by label \textbf{l1}, into two separate for-loops, \textbf{l2} and
\textbf{l3}. We apply this to PageRankDelta in Listing~\ref{lst:kernel_split}. The first split loop's range goes from 1--4 and the
second one from 4 to 11.  For the first 4 iterations, the program
simply uses DensePull, whereas for later iterations the program uses
DensePull-SparsePush. This reduces unnecessary work in the first
several iterations for computing the sum of out-degrees. 

\begin{lstlisting} [language=graphit, caption={Kernel split}, label={lst:kernel_split}, escapechar=|]
...
#l1# for i in 1:11
	#s1# edges.from(frontier).apply(updateEdge);
	...
end
...
schedule:
program
->splitForLoop("l1", "l2", "l3", 3, 7);
->configApplyDirection("l2:s1", "DensePull")
->configApplyParallelization("l2:s1", "vertex-parallel");
->configApplyDirection("l3:s1", "DensePull-SparsePush")
->configApplyParallelization("l3:s1", "vertex-parallel");
->fuseFields("Delta", "OutDegree");
\end{lstlisting}

}

\punt{
\myparagraph{Splitting iterative graph kernels} The performance of
iterative graph kernels can be further improved by providing the user with the
ability to specify different schedules for different iterations of the
program.  For example, the first several iterations of PageRankDelta
usually have a large active set (frontier) and a DensePull traversal
is efficient, whereas later iterations have a smaller active set
and a SparsePush traversal avoids unnecessary edge traversals. 
Programmers can use \splitForLoop{} and scoped labels to 
schedule the outer for loop with DensePull for 
the first few iterations and DensePull-SparsePush for later iterations. 
This schedule reduces the overhead in computing the sum of out-degrees, 
which can be quite  significant for certain graphs.




\riyadh{The purpose of the following section is not clear to me. Does it talk
about the three categories of optimizations ? or about how we
implement them ? or about we represent them ? The first subsubsection (edge
	traversal optimizations) seems to focus on the representation (GIS) while
	the other subsubsections (data layout and multiedge) seem to focus
	on describing how we implement the optimization. I think the last two subsubsections
	(data layout and multiedge transversal) can be improved by talking
	more about the "representation" (or maybe just say a sentence in
     their beginning in which you mention the word "representation", that would
    remind the reader that this is about the representation}
}




==> schedule_rep_stash.tex <==
\punt{
\graphit introduces three categories of optimizations
---\textit{Single Edge Traversal Optimizations}, \textit{Vertex Data
Layout Optimizations}, and \textit{Multiple Edge Traversals Optimizations} as shown in Figure~\ref{fig:GIS_supported}. 
}

\punt{
Performing and composing edge traversal optimizations in the general
case is challenging because it requires the ability to represent the original
code, the ability to express and compose code optimizations and the ability
to reason about the correctness of the optimizations.
The question is then: How can the \graphit compiler represent the code and
represent the code optimizations in a way that allows the composition
of transformations ? And how can the \graphit compiler guarantee
the correctness of code transformations ? To solve these problems we
introduce the \textit{Graph Iteration Space}.  We use the graph iteration
space as an abstract representation of the code; Edge traversal optimizations
are expressed as transformations of this iteration space and this simplifies
the composition of transformations.  We also use the graph iteration space
to perform dependence analysis.  We use the dependence analysis to guarantee
the correctness of parallelization (insert synchronization when necessary).
}

\punt{
A new dimension in the dense loop iteration is created with blocking or partitioning the loops, 
a new dimension in graph iteration space is created by partitioning a new subgraph. 
This can be achieved through both program and edge data transformations. 
Adding new dimensions to the graph 
graph iteration space can optimize the locality and load balance of the applications, 
while incurring additional work overhead. 
Compared to the traditional dense iteration space, 
graph iteration space is sparse, containing only pairs in the edge set, and supports filtering on the source and destinations. 
For a given source $src$, there is no duplication among $dst$'s  (no duplicate edges), no $dst$ that is the same as $src$ (no self loops), and no order among the $dst$'s.

}


\punt{

More precisely, the graph iteration space of \textbf{L} is defined as the
set of tuples $\langle Segmented Subgraph (SSG), Blocked Subgraph (BSG),  OuterIter, InnerIter \rangle$ where each tuple represents an edge. 
The source $src$ is in the filtered source vertexset of \textbf{L} (specified with
 the~\from~and~\srcFilter~ operators on \textbf{L}), the destination $dst$ is in the
filtered destination vertexset of \textbf{L} (specified with the \too{} and
\dstFilter{} operators on \textbf{L}), and the edge $(src, dst)$ is in
the edge set of $sg$.
If the graph is partitioned, then $sg$ represents one of the subgraphs
(partitions) of the original graph otherwise it represents the original
graph.  


%show the limited graph iteration space
\begin{footnotesize}
\vspace{-4pt}
\begin{equation*}
\left\{\begin{tabular}{c|c}
				       & $src$ $\in$ filtered source vertex set of \textbf{L}\\ 
	$\langle sg, src, dst \rangle$ & $dst$ $\in$ filtered destionation vertex set of \textbf{L}\\ 
				       & $\langle$ src, dst $\rangle \in$ edge set of $sg$
\end{tabular}\right\}	
\end{equation*}
\vspace{-4pt}
\end{footnotesize}

}

==> tradeoff_stash.tex <==
\section{Tradeoff Space and Optimizations}
\label{sec:tradeoff}

% We examine the challenges in writing a high performance graph application
% optimization techniques developed for graphs
% programming models 

In this section, we describe the tradeoff space for optimizing graph
programs.  While the effects of various optimizations are well-known
to expert programmers, we believe that we are the first to
characterize this optimization tradeoff space. Our tradeoff space
consists of three properties of graph programs---locality, work, and
parallelism. \defn{Locality} refers to the amount of spatial and
temporal reuse in a program. Increasing the amount of resuse improves
locality due to increasing the number of cache hits.  \defn{Work}
refers to the total number of instructions executed where each type of
instruction is weighted according to its execution time. Reducing work
improves performance.  \defn{Parallelism} refers to the relative
amount of work that can be executed independently by different
processing units. Increasing parallelism improves performance by
taking advantage of more processing units, and helping to hide the
latency of DRAM requests.  As we will see, each optimization can
affect multiple factors of a program, either positively or negatively.
The complex tradeoff space motivates the design of \graphit's
scheduling language and compiler, which can be used to easily search
for points in the tradeoff space that achieve high performance.

\input{opt-table}

\subsection{PageRankDelta}
We describe how the optimizations fit into the tradeoff space using
PageRankDelta~\cite{shun13ppopp-ligra}, but note that these
optimizations are applicable to other graph algorithms as
well. PageRankDelta is a variant of the standard PageRank
algorithm~\cite{page99tr-pagerank} that computes the importance of
vertices in a graph. It maintains an array of ranks, and on each
iteration, updates the ranks of all vertices based on the ranks of
their neighbors weighted by their neighbors'
out-degrees. PageRankDelta speeds up the computation by updating only
the ranks of vertices whose ranks have changed significantly from the
previous iteration.

\algrenewcommand{\alglinenumber}[1]{\footnotesize#1}

\algdef{SE}[SUBALG]{Indent}{EndIndent}{}{\algorithmicend\ }%
\algtext*{Indent}
\algtext*{EndIndent}
%\algnewcommand\algorithmicparfor{\textbf{parfor}}

%% \algdef{SE}[PARFOR]{ParFor}{EndFor}[1]{\algorithmicparfor\ #1\ \algorithmicdo}{\algorithmicend\ \algorithmicfor}%

\algblockdefx[pfor]{ParFor}{EndParFor}[1]
  {\textbf{parallel for}~#1~\textbf{do}}{}
  
\algtext*{EndParFor}

\begin{algorithm}[t]
\caption{PageRankDelta (SparsePush)}
\label{alg:PageRankDelta}
\begin{algorithmic}[1]
\scriptsize 

%\State typedef double vertexDataType
\State Rank $=  \{0, \ldots, 0\}$ \Comment{Length $V$ array}
\State DeltaSum $=  \{0.0, \ldots, 0.0\}$ \Comment{Length $V$ array} 
\State Delta $= \{1/V, \ldots, 1/V\}$ \Comment{Length $V$ array}
%% \State Damping $= 0.85$
%% \State Epsilon $= 0.01$
\smallskip
\Procedure{PageRankDelta}{Graph $G$, $\alpha$, $\epsilon$}
	\State Frontier = $\{$ $G$.vertices $\}$ \label{line:init-frontier}
	\For {round $\in\{1,\ldots,$MaxIter$\}$}
		\State NextFrontier = $\{ \}$
		\ParFor{src : Frontier} \label {line:access_src}
			\For{dst : $G$.getOutNgh[src]} \label {line:access_dst} %\Comment{Parallel for high-degree vertices}
				\State DeltaSum[dst] $\mathrel{+}=$ Delta[src] $/$ G.OutDegree[src] \label{line:update_dst} \Comment{Atomic}
			\EndFor
		\EndParFor
		\ParFor {v : $G$.vertices} \label{line:start_delta_comp}
			\If {round $== 1 $}
				\State BaseScore $=(1.0 - \alpha)/V$ 
				\State Delta[v] $= \alpha \cdot ($DeltaSum[v]$) +$ BaseScore
				\State Delta[v] $\mathrel{-}= 1/V$      
			\Else {} 
				\State Delta[v] $= \alpha  \cdot ($DeltaSum[v]$)$
			\EndIf
			\State Rank[v] $\mathrel{+}=$ Delta[v] \label{line:end_delta_comp}
			\State DeltaSum[v] $=$ 0 
			\If {$\mid$Delta[v]$\mid > \epsilon \cdot $Rank[v]} \label{line:vertex_filtering}
				\State NextFrontier.add(v) \label{line:filling_frontier}
			\EndIf
		\EndParFor \label{line:end_vertex_filtering}
		\State Frontier $=$ NextFrontier
	\EndFor \label{line:done}
\EndProcedure
\end{algorithmic}
\end{algorithm}

The pseudocode for PageRankDelta is shown in
Algorithm~\ref{alg:PageRankDelta}, where $V$ is the number of vertices
in the graph, $0 \leq \alpha \leq 1$ is the damping factor that determines how heavily to weight the neighbors' ranks during the update, and $\epsilon \geq 0$ is a constant that determines whether a vertex's rank has changed sufficiently.
For simplicity we update the ranks of vertices for
MaxIter number of iterations, although the code can easily be
modified to terminate based on a convergence criteria. The algorithm
maintains the set of vertices whose ranks (stored in the Rank array) have changed significantly
from the previous iteration in the variable Frontier. We will refer to
this as the \emph{active set} of vertices or the \emph{frontier}.  Initially all vertices are in the active set (Line~\ref{line:init-frontier}). On each iteration, each
vertex in the active set sends its Delta (change in Rank value) from the
previous iteration to its out-neighbors by incrementing the DeltaSum values
of its neighbors
(Lines~\ref{line:access_src}--\ref{line:update_dst}). Since vertices
are processed in parallel, the update to DeltaSum has to be atomic.
Then in parallel, all vertices compute their own Delta and Rank values based on
its DeltaSum value and $\alpha$
(Lines~\ref{line:start_delta_comp}--\ref{line:end_delta_comp}).  The
Delta is computed differently for the first iteration.  If the Delta
of the vertex is larger than $\epsilon$ times its Rank, then the vertex
is active for the next iteration and gets added to the next frontier
(Lines~\ref{line:vertex_filtering}--\ref{line:end_vertex_filtering}).

%The algorithm repeat itself for max iterations.
%% PageRankDelta's iterative and data-driven nature is representative of important graph applications, such as Breadth-First Search and Connected Components. 
%% It also exposes issues present in applications that do not use active vertex tracking including PageRank and Collaborative Filtering.

%\subsection{Performance Tradeoff Space}

%% \begin{figure}[t]
%% \includegraphics[width=\columnwidth]{figures/tradeoff_axis}	
%% \caption{Performance Tradeoff Space and Optimizations}
%% \label{fig:tradeoff_space}
%% \end{figure}

% Graph application is bottlenecked on memory subsystem
%% \myparagraph{Locality} Improving the locality of memory accesses is critical for graph applications. 
%% For example, the PageRankDelta algorithm loops over all vertices in the frontier in each iteration, and for each source vertex reads and writes the DeltaSum of
%% its neighbors (lines~\ref{line:access_dst} to~\ref{line:update_dst}). Since the neighbors of a vertex can be arbitrary (input
%% dependent), accesses to the fields of neighbors have very poor locality. 
%% The datasets (DeltaSum) are often many times the size of the last level cache
%% (LLC), a large portion of the random requests goes to DRAM directly. 
%% Since accesses to DRAM can take hundreds of cycles, the application is often stalled on memory requests. The read and writes to neighbor DeltaSum can take up to 80$\%$ of the overall execution time. \julian{Is this number for PageRank or PageRankDelta? Add citation.}

%% \myparagraph{Parallelism} Exploiting parallelism is important for graph applications to achieve good performance. For PageRankDelta, the read and writes to neighbors' DeltaSum (lines~\ref{line:access_src} to ~\ref{line:update_dst}) and computing the updated Delta (lines~\ref{line:start_delta_comp} to ~\ref{line:end_delta_comp}) can be done in parallel with with some synchronizations.

%% \myparagraph{Work-Efficiency} It is important to minimize the number of random memory accesses and extra work incurred by graph optimizations.

\subsection{Graph Optimizations}
We will describe how different optimizations can be applied to
PageRankDelta.  For reference, Table~\ref{table:opt-table} contains
the various optimizations considered in this paper, as well as their
effects on the different characteristics of a program. We analyze the
effect of optimizations relative to the baseline in
Algorithm~\ref{alg:PageRankDelta}, which we refer to as
\emph{SparsePush}.

\myparagraph{Edge Traversal Optimization}
Lines~\ref{line:access_src}--\ref{line:update_dst} of SparsePush
iterate over the outgoing neighbors of each vertex, and update the
DeltaSum value of the neighbor. Another way to perform this
computation is to have each vertex iterate over its incoming neighbors
that are in the active set, and update its own DeltaSum value. We
refer to this method as \emph{DensePull} and the pseudocode for the
part of the program computing DeltaSum using this method is shown in
Algorithm~\ref{alg:PageRankDeltaPull}.  DensePull increases
parallelism relative to SparsePush since it loops over all
vertices. Looping over all vertices causes its work to increase
(SparsePush only needs to loop over vertices in the active set), but
the overall number of edges traversed could increase or decrease.  The
update to the DeltaSum array no longer requires atomics since an entry
will not be updated in parallel, and this reduces synchronization
overhead. Instead of doing random writes as in SparsePush, DensePull does random reads and mostly sequential writes, which are cheaper. For some algorithms (e.g., breadth-first search), the inner loop over the in-neighbors in DensePull
can exit early to reduce overall work. A detailed performance study of the two traversal methods can be found in~\cite{Besta2017}.

\punt{
% this is a bit tricky to explain without a detailed exampel
(e.g., after finding one in-neighbor on the frontier in
breadth-first search), which
}

\begin{algorithm}[t]
\caption{DensePull}
\label{alg:PageRankDeltaPull}
\begin{algorithmic}[1]
\scriptsize 
\ParFor{dst : $G$.vertices} \label {line:pull_access_dst}
			\For{src : $G$.getInNgh[dst]} \label {line:pull_access_src}
				\If{src $\in$ Frontier}
					\State DeltaSum[dst] $\mathrel{+}=$ Delta[src] $/$ G.OutDegree[src] \label{line:pull_update_dst}
				\EndIf
			\EndFor
			%\State Compute new Delta, Rank for and update Frontier
\EndParFor
\end{algorithmic}
\end{algorithm}

One could also implement the computation of DeltaSum by looping
through all vertices and checking if each one is on the frontier
instead of just looping over frontier vertices. We call this version \emph{DensePush}
(Algorithm~\ref{alg:PageRankDeltaDensePush}). While iterating over all
vertices increases work, this could be offset by not having to
maintain the frontier in a sparse format. The updates have to be
atomic, which increases synchronization overhead.

\begin{algorithm}[t]
\caption{DensePush}
\label{alg:PageRankDeltaDensePush}
\begin{algorithmic}[1]
\scriptsize 
\ParFor{src : $G$.vertices} \label {line:dense_push_access_src}
		\If{src $\in$ Frontier} \label {line:dense_push_check_src}
			\For{dst : $G$.getOutNgh[src]} \label {line:dense_push_access_dst} %\Comment{Parallel for high-degree vertices}
					\State DeltaSum[dst] $\mathrel{+}=$ Delta[src] $/$ G.OutDegree[src] \Comment{Atomic} \label{line:pull_update_dst}
			\EndFor
		\EndIf
\EndParFor
\end{algorithmic}
\end{algorithm}


%% Algorithm~\ref{alg:PageRankDeltaPull} shows a push mode that loops through the active vertices on
%% the current frontier / active set (Algorithm~\ref{alg:PageRankDelta} line 12), and accesses data
%% associated with their outgoing edge neighbors (Algorithm~\ref{alg:PageRankDelta} lines~\ref{line:access_dst} to ~\ref{line:update_dst}). 
%% In the pull mode, the outer loop
%% goes through all vertices and checks if there is
%% a incoming edge neighbor on the frontier that can update it (Algorithm~\ref{alg:PageRankDeltaPull} lines~\ref{line:pull_access_dst} to ~\ref{line:pull_update_dst}). 
%which optimizations to discuss?
% direction optimization, parallelization, load balance, bitvector, AoS vs SoA, Split?
%% Many graph optimizations have been proposed as points in the tradeoff space. Here we discuss a few important effective optimizations, edge traversal direction optimization, including parallelization and data layout optimizations.


%% \myparagraph{Edge Traversal Direction Optimization} Optimizing edge
%% traversal direction can also play a big role in the work-efficiency and parallelism aspects of the program~\cite{Beamer-2012, shun13ppopp-ligra}. 
%% \punt{
%%  This idea was first proposed by Beamer et al.~\cite{Beamer-2012} to reduce the number of random accesses
%% for BFS, and was later generalized to other graph traversal algorithms
%% by Ligra~\cite{shun13ppopp-ligra}.}

%% Generally speaking, there can be two directions for traversing the edges, top-down (push) and bottom-up (pull). Later we show how it can be further divided into a dense and sparse variant of each direction.
%% Algorithm~\ref{alg:PageRankDelta} shows a push mode that loops through the active vertices on
%% the current frontier / active set (Algorithm~\ref{alg:PageRankDelta} line 12), and accesses data
%% associated with their outgoing edge neighbors (Algorithm~\ref{alg:PageRankDelta} lines~\ref{line:access_dst} to ~\ref{line:update_dst}). 
%% In the pull mode, the outer loop
%% goes through all vertices and checks if there is
%% a incoming edge neighbor on the frontier that can update it (Algorithm~\ref{alg:PageRankDeltaPull} lines~\ref{line:pull_access_dst} to ~\ref{line:pull_update_dst}). 

% If we have to cut some space, it might be good to cut the dense push algorithm and description

A program can be designed to use different traversal modes
(SparsePush, DensePull, DensePush) in different iterations based on
the size of the active set. This idea was explored
in~\cite{Beamer-2012,shun13ppopp-ligra} to reduce overall work by
reducing edge traversals, random writes, and synchronization overheads.

In PageRankDelta, the number of vertices in the frontier
gradually decreases as the ranks of vertices starts to converge. In
the early iterations, DensePull is preferred due to lower
synchronization overheads and avoiding random writes.  As the frontier
shrinks, SparsePush is preferred due to the fewer number of vertices
that need to be traversed. A hybrid scheme for computing the DeltaSum
values in PageRankDelta computes the sum of out-degrees of the
frontier vertices and uses DensePull if the sum is above some
threshold, and SparsePush otherwise. We call this version
\emph{DensePull-SparsePush}. For some algorithms, DensePush can
perform better than DensePull, which leads to another hybrid version
\emph{DensePush-SparsePush}. There is additional work in the
hybrid versions to compute the sum of out-degrees of the vertices
in the active set, which can have significant overhead for some graphs.


%% doing a push traversal would need only to access 
%% a much smaller subgraph, versus a pull direction traversal would still need to access the entire graph.
%% The direction optimization can also impact atomic
%% synchronization overheads, since no atomics are needed when using the
%% the pull mode (updates to a dst are done sequentially in Algorithm~\ref{alg:PageRankDeltaPull} line~\ref{line:pull_update_dst}). The push mode would need atomic updates to the DeltaSum of the destination (Algorithm~\ref{alg:PageRankDelta} line~\ref{line:update_dst}). As a result, in the first few iterations, it makes sense to perform the computation in pull direction.

% as shown in Algorithm~\ref{alg:PageRankDeltaDensePush}
%% Each direction can be further divided in a sparse and dense variant.
%% For example, Algorithm\ref{alg:PageRankDelta} shows a sparse push variant, where the outer loop traverses 
%% through only vertices on the frontier (active vertices). 
%% A dense version can traverse through all the vertices and check if the current vertex is on the frontier. The dense push version can be more effective than the sparse push version by exploiting more parallelism, reducing the cost needed to compute a dense version of the frontier. 
%% However, the unnecessary checks in line~\ref{line:dense_push_access_dst} can hurt work-efficiency. 
%% The pull version can also have the two variants when a frontier for destination vertices is specified.

%% \begin{algorithm}[t]
%% \caption{PageRankDelta-Hybrid}
%% \label{alg:PageRankDeltaHybrid}
%% \begin{algorithmic}[1]
%% \scriptsize 
%% 	\State OutDegreeSum = 0 \label{line:degree_compute_start}
%% 	\For{src : Frontier}
%% 		\State OutDegreeSum $\mathrel{+}=$ G.OutDegree[src]
%% 	\EndFor \label{line:degree_compute_end}
%% 	\If {OutDegreeSum $>$ threshold}
%% 		\State Do Traversal Mode 1 
%% 	\Else {}
%% 		\State Do Traversal Mode 2
%% 	       \EndIf
%% \EndFor

%% \end{algorithmic}
%% \end{algorithm}


%% A
%% hybrid scheme (Algorithm~\ref{alg:PageRankDeltaHybrid}) that switches between two different modes based on the sum of OutDegrees of vertices on the frontier
%% size can lead to significant savings of number of random memory accesses, at a cost of extra computations (lines~\ref{line:degree_compute_start} to ~\ref{line:degree_compute_end}). 
%% For graphs
%% where one mode is always better than the other, this extra sum of OutDegrees computation can lead
%% to significant performance degradation.


\myparagraph{Parallelization and Load Balance}
%% Since graph algorithms often have a large degree of data parallelism, it is important to achieve good scalability for high performance implementations. Parallelism can also help hide the long latency DRAM requests by issuing a large number memory requests. 
For each traversal mode, there are different methods for parallelization. The parallelization shown in Algorithms~\ref{alg:PageRankDelta}--\ref{alg:PageRankDeltaDensePush} processes the vertices in parallel (using a work-stealing scheduler). 
%% There are several parallelization choices for graph algorithms. The most commonly adopted approach uses work-stealing based vertex level parallelism, which replaces the sequential for loop line~\ref{line:access_src} in Algorithm~\ref{alg:PageRankDelta} and line~\ref{line:pull_access_dst} in Algorithm~\ref{alg:PageRankDeltaPull} with parallel for loop and insert synchronizations.
This approach, which we call \emph{vertex-parallel}, works reasonably
well on a number of applications where the workload of each vertex is
similar. However, for skewed degree distributions, this approach can
lead to significant load imbalance.  For these workloads, an
edge-aware vertex-parallel scheme (which we refer to as
\emph{edge-aware-vertex-parallel}) can be more effective.  This
approach uses a divide-and-conquer scheme to break up the vertices
into a number of vertex chunks, where each chunk has approximately the
same number of edges, improving load balance across different chunks,
which improves parallelism. However, this scheme incurs additional
work for computing the sum of degrees of vertices in each chunk.
Finally, we can parallelize across all edges, instead of just
vertices, by parallelizing the inner loop of the edge-traversal code
computing DeltaSum in
Algorithms~\ref{alg:PageRankDelta}--\ref{alg:PageRankDeltaDensePush}. We
refer to this method as \emph{edge-parallel}. This improves
parallelism but increases work due to the overhead of work-stealing in
the inner loop, requiring atomic updates for DensePull, and disabling
early breaking of the inner loop for DensePull. 

\punt{ More sophisticated
schemes for Edge-parallel can be implemented, such as only
parallelizing across edges for high-degree vertices, and for DensePull
parallelizing across edges in chunks and checking the early break
condition after each chunk.}


\begin{algorithm}[t]
\caption{DensePull with Data Layout Optimizations}
\label{alg:PageRankDeltaPullBitvectorWithStructs}
\begin{algorithmic}[1]
\scriptsize 
\State Bitvec = ConvertToBitvec(Frontier)\label{line:pull_opt_setup_bitvec}
\ParFor{dst : $G$.vertices} \label {line:pull_access_dst}
			\For{src : $G$.getInNgh[dst]} \label {line:pull_access_src}
				\If{Bitvec.getBit(src)} \label{line:pull_opt_use_bitvec}
					\State DeltaSum[dst] $\mathrel{+}=$ FusedStruct[src].Delta$/$FusedStruct[src].OutDegree\label{line:pull_opt_update_dst}
				\EndIf
			\EndFor
\EndParFor
\end{algorithmic}
\end{algorithm}

\myparagraph{Data Layout Optimizations} The layout of data can greatly
affect the locality of memory accesses. One optimization to improve
locality is to use bitvectors instead of boolean arrays to keep track
of vertices on the frontier for the dense traversal modes. This
improves spatial locality, but requires extra work to compress the
boolean array and access it.  We refer to this optimization as \emph{bitvector}.

Furthermore, random accesses to the same index of two separate arrays
(e.g., the Delta and OutDegree arrays in PageRankDelta) can be changed
into a single random access to an array of structs to improve spatial
locality.  However, grouping together fields that are not always
accessed together expands the working set and hurts the locality of
the data structures. Converting between array of structs and struct of
arrays (we refer to this optimization as \emph{AoS-SoA}) requires
extra work, although this cost is usually small compared to the rest
of the algorithm.  The pseudocode of the portion of PageRankDelta
computing DeltaSum using the DensePull traversal and using the two
data layout optimizations is shown in
Algorithm~\ref{alg:PageRankDeltaPullBitvectorWithStructs}.

%% For example, boolean arrays used to keep track of vertices on the frontier can be compressed into bitvectors, reducing the working set size by 32x and boosting spatial locality (Algorithm~\ref{alg:PageRankDeltaPullBitvectorWithStructs} lines~\ref{line:pull_opt_setup_bitvec},~\ref{line:pull_opt_use_bitvec}). However, the penalty on work-efficiency with extra instructions to compress the boolean array at runtime might outweigh the gains in locality.

%% Random accesses to the same index of two separate arrays (Delta, OutDegree) can be changed
%% into a single random access to an array of structs to further improve the spatial locality of the vertex data structures (Algorithm~\ref{alg:PageRankDeltaPullBitvectorWithStructs} line~\ref{line:pull_opt_update_dst}).  

\myparagraph{Program structure transformations} The \emph{kernel split}
optimization splits a loop in a program into multiple loops, which can
be useful if the programmer knows when certain iterations are always
more efficient with a particular traversal mode. This allows
the resulting loops to always use a certain traversal method, reducing
the work incurred from the hybrid method for computing the sum of
out-degrees.
%% For example, this can be used for the first round of
%% PageRankDelta since the active set always contains all vertices.

When two graph kernels have the same traversal pattern (they process
the same vertices/edges on each iteration), we can fuse the kernels
together by fusing their data structures into an array of structs and
fusing the updates they apply to the vertices. We refer to this optimization
as \emph{kernel fusion}. This improves spatial locality by enabling
the program to access the fields of the two kernels together when
traversing the edges. Additional work is incurred for performing the
AoS-SoA optimization, but again this is usually small compared to the
rest of the algorithm.




% We examine the challenges in writing a high performance graph application
% optimization techniques developed for graphs
% programming models 


%The algorithm repeat itself for max iterations.
%% PageRankDelta's iterative and data-driven nature is representative of important graph applications, such as Breadth-First Search and Connected Components. 
%% It also exposes issues present in applications that do not use active vertex tracking including PageRank and Collaborative Filtering.

%\subsection{Performance Tradeoff Space}

%% \begin{figure}[t]
%% \includegraphics[width=\columnwidth]{figures/tradeoff_axis}	
%% \caption{Performance Tradeoff Space and Optimizations}
%% \label{fig:tradeoff_space}
%% \end{figure}

% Graph application is bottlenecked on memory subsystem
%% \myparagraph{Locality} Improving the locality of memory accesses is critical for graph applications. 
%% For example, the PageRankDelta algorithm loops over all vertices in the frontier in each iteration, and for each source vertex reads and writes the DeltaSum of
%% its neighbors (lines~\ref{line:access_dst} to~\ref{line:update_dst}). Since the neighbors of a vertex can be arbitrary (input
%% dependent), accesses to the fields of neighbors have very poor locality. 
%% The datasets (DeltaSum) are often many times the size of the last level cache
%% (LLC), a large portion of the random requests goes to DRAM directly. 
%% Since accesses to DRAM can take hundreds of cycles, the application is often stalled on memory requests. The read and writes to neighbor DeltaSum can take up to 80$\%$ of the overall execution time. \julian{Is this number for PageRank or PageRankDelta? Add citation.}

%% \myparagraph{Parallelism} Exploiting parallelism is important for graph applications to achieve good performance. For PageRankDelta, the read and writes to neighbors' DeltaSum (lines~\ref{line:access_src} to ~\ref{line:update_dst}) and computing the updated Delta (lines~\ref{line:start_delta_comp} to ~\ref{line:end_delta_comp}) can be done in parallel with with some synchronizations.

%% \myparagraph{Work-Efficiency} It is important to minimize the number of random memory accesses and extra work incurred by graph optimizations.


\punt{
  % this is a bit tricky to explain without a detailed exampel
  (e.g., after finding one in-neighbor on the frontier in
  breadth-first search), which }

%% For example, boolean arrays used to keep track of vertices on the
%% frontier can be compressed into bitvectors, reducing the working
%% set size by 32x and boosting spatial locality
%% (Algorithm~\ref{alg:PageRankDeltaPullBitvectorWithStructs}
%% lines~\ref{line:pull_opt_setup_bitvec},~\ref{line:pull_opt_use_bitvec}). However,
%% the penalty on work-efficiency with extra instructions to compress
%% the boolean array at runtime might outweigh the gains in locality.

%% Random accesses to the same index of two separate arrays (Delta,
%% OutDegree) can be changed into a single random access to an array
%% of structs to further improve the spatial locality of the vertex
%% data structures
%% (Algorithm~\ref{alg:PageRankDeltaPullBitvectorWithStructs}
%% line~\ref{line:pull_opt_update_dst}).



%% doing a push traversal would need only to access a much smaller
%% subgraph, versus a pull direction traversal would still need to
%% access the entire graph.  The direction optimization can also
%% impact atomic synchronization overheads, since no atomics are
%% needed when using the the pull mode (updates to a dst are done
%% sequentially in Algorithm~\ref{alg:PageRankDeltaPull}
%% line~\ref{line:pull_update_dst}). The push mode would need atomic
%% updates to the DeltaSum of the destination
%% (Algorithm~\ref{alg:PageRankDelta} line~\ref{line:update_dst}). As
%% a result, in the first few iterations, it makes sense to perform
%% the computation in pull direction.

% as shown in Algorithm~\ref{alg:PageRankDeltaDensePush}
%% Each direction can be further divided in a sparse and dense
%% variant.  For example, Algorithm\ref{alg:PageRankDelta} shows a
%% sparse push variant, where the outer loop traverses through only
%% vertices on the frontier (active vertices).  A dense version can
%% traverse through all the vertices and check if the current vertex
%% is on the frontier. The dense push version can be more effective
%% than the sparse push version by exploiting more parallelism,
%% reducing the cost needed to compute a dense version of the
%% frontier.  However, the unnecessary checks in
%% line~\ref{line:dense_push_access_dst} can hurt work-efficiency.
%% The pull version can also have the two variants when a frontier for
%% destination vertices is specified.

%% \begin{algorithm}[t]
%%   \caption{PageRankDelta-Hybrid}
%%   \label{alg:PageRankDeltaHybrid}
%%   \begin{algorithmic}[1]
%%     \scriptsize \State OutDegreeSum =
%%     0 \label{line:degree_compute_start} \For{src : Frontier} \State
%%     OutDegreeSum $\mathrel{+}=$ G.OutDegree[src]
%%     \EndFor \label{line:degree_compute_end} \If {OutDegreeSum $>$
%%     threshold} \State Do Traversal Mode 1 \Else {} \State Do
%%     Traversal Mode 2 \EndIf \EndFor

%%   \end{algorithmic}
%% \end{algorithm}


%% A hybrid scheme (Algorithm~\ref{alg:PageRankDeltaHybrid}) that
%% switches between two different modes based on the sum of OutDegrees
%% of vertices on the frontier size can lead to significant savings of
%% number of random memory accesses, at a cost of extra computations
%% (lines~\ref{line:degree_compute_start} to
%% ~\ref{line:degree_compute_end}).  For graphs where one mode is
%% always better than the other, this extra sum of OutDegrees
%% computation can lead to significant performance degradation.

\punt{ % not show the last bit of pseudo code to save space
The pseudocode of the portion
of PageRankDelta computing DeltaSum using the DensePull traversal and
using the vertex data layout optimization is shown in
Fig.~\ref{alg:PageRankDeltaPullBitvectorWithStructs}.
}



\punt{
Converting between array of structs (AoS) and struct of
arrays (SoA) requires extra work, although this cost is usually small
compared to the rest of the algorithm.  }


\punt{

  \myparagraph{Program structure transformations} The \emph{kernel
    split} optimization splits a loop in a program into multiple
  loops, which can be useful if the programmer knows when certain
  iterations are always more efficient with a particular traversal
  mode. This allows the resulting loops to always use a certain
  traversal method, reducing the work incurred from the hybrid method
  for computing the sum of out-degrees.
  %% For example, this can be used for the first round of
  %% PageRankDelta since the active set always contains all vertices.

  When two graph kernels have the same traversal pattern (they process
  the same vertices/edges on each iteration), we can fuse the kernels
  together by fusing their data structures into an array of structs
  and the updates they apply to the vertices. We refer to this
  optimization as \emph{kernel fusion}. This improves spatial locality
  by enabling the program to access the fields of the two kernels
  together when traversing the edges. Additional work is incurred for
  performing the vertex data layout optimization, but again this is
  usually small compared to the rest of the algorithm.  }


